On groups with few subgroups not in the Chermak-Delgado lattice

We investigate the question of how many subgroups of a finite group are not in its Chermak-Delgado lattice. The Chermak-Delgado lattice for a finite group is a self-dual lattice of subgroups with many intriguing properties. Fasol\u{a} and T\u{a}rn\u{a}uceanu asked how many subgroups are not in the Chermak-Delgado lattice and classified all groups with two or less subgroups not in the Chermak-Delgado lattice. We extend their work by classifying all groups with less than five subgroups not in the Chermak-Delgado lattice. In addition, we show that a group with less than five subgroups not in the Chermak--Delgado lattice is nilpotent. In this vein we also show that the only non-nilpotent group with five or fewer subgroups in the Chermak-Delgado lattice is S_3.

==> cocke_code/check_conds1_2.tex <==
\begin{verbatim}
H_in_cd:=function(H)
       cd_H := Max([#K`subgroup*#Centralizer(H,K`subgroup): K in Subgroups(H)]);
       return #H*#Center(H) eq cd_H;
end function;

not_in_cd:=function(H)
      cd_H := Max([#K`subgroup*#Centralizer(H,K`subgroup): K in Subgroups(H)]);
      if #CD_H eq 0 then return 0; end if;
      return &+CD_H;
end function;

order := 32;
Y := {};
X := {};
ZZ := {x: x in [1..NumberOfSmallGroups(order)]|
H_in_cd(SmallGroup(order,x)) and not_in_cd(SmallGroup(order,x)) lt 1};
for i in [1..NumberOfSmallGroups(order)] do
    K:=SmallGroup(order,i);
    Z:=Center(K);
    for H in Subgroups(Z:OrderEqual:=2) do
        if #{*1: J in Subgroups(K)|J`order ge 4 
        and (#sub<K|J`subgroup,H`subgroup> ne #sub<K|J`subgroup>)*} gt 1 
        then continue; end if;
        Include(~X,i);
    end for;
    if #{x: x in K | Order(x) eq 2} le 3 then Include(~Y,i); end if;
end for;
X;
Y;
ZZ;
X meet Y meet ZZ;

order := 243;
Y := {};
X := {};
ZZ := {x: x in [1..NumberOfSmallGroups(order)]|
H_in_cd(SmallGroup(order,x)) and not_in_cd(SmallGroup(order,x)) lt 1};
for i in [1..NumberOfSmallGroups(order)] do
    K:=SmallGroup(order,i);
    Z:=Center(K);
    for H in Subgroups(Z:OrderEqual:=2) do
        if #{*1: J in Subgroups(K)|J`order ge 4 
        and (#sub<K|J`subgroup,H`subgroup> ne #sub<K|J`subgroup>)*} gt 1 
        then continue; end if;
        Include(~X,i);
    end for;
    if #{x: x in K | Order(x) eq 2} le 3 then Include(~Y,i); end if;
end for;
X;
Y;
ZZ;
X meet Y meet ZZ;
\end{verbatim}

==> lemma_5_3.tex <==
\section*{Appendix A}
\textsc{GAP} code used to prove Lemma \ref{lem: 32} and \ref{thm: lt53}.
\begin{verbatim}
#compute the Chermak-Delgado measure of K in H
CD_measure:=function(H,K)
return Order(K)*Order(Centralizer(H,K));
end;

#compute m^*(H)
Max_CD_measure:=function(H)
return MaximumList(List(ConjugacyClassesSubgroups(H),x->CD_measure(H,Representative(x))));
end;

#check to see if $H \in CD(H)$
H_in_CDL:=function(H)
	if CD_measure(H,H) = Max_CD_measure(H) then
		return true;
	else
		return false;
	fi;
end;

#count the number of subgroups not in the CD Lattice(H) which contain Z(H)


NumberSubgroupsContainingCenterOutsideCDL:=function(H)
  local toCount, SubgroupConjugacyClasses, max_cdm, Z_H, rep, class;

toCount:=[];
SubgroupConjugacyClasses:=ConjugacyClassesSubgroups(H);
max_cdm:=Max_CD_measure(H);
Z_H:=Center(H);

for class in SubgroupConjugacyClasses do
	rep:=Representative(class);
		if CD_measure(H,rep) <> max_cdm and IsSubset(rep,Z_H) then
			Add(toCount,class);
		fi;
od;

return Sum(List(toCount,x->Size(x)));
end;

NumberSubgroupsOrder_p:=function(H)
  local p, classes_order_p;

p:=PrimePGroup(H);
classes_order_p:=Filtered(ConjugacyClasses(H),x->Order(Representative(x))=2);
return Sum(List(classes_order_p,x->Size(x)));
end;

NumberSubgroupsNotContainingCentralSubgroup:=function(K,Z)
  local p, toCount, rep, class;

#we assume $Z <= Z(K)$
#we count the number of subgroups of $K$ of order >= p^2 which do not contain Z
#we can do this by identifying the conjugacy classes which do or do not contain
#Z as a subgroup and then count the lengths of the conjugacy classes which do not

p:=PrimePGroup(K);
toCount:=[];
for class in Filtered(ConjugacyClassesSubgroups(K), x->Order(Representative(x))>= p^2) do
	rep:=Representative(class);
		if not IsSubset(rep,Z) then
			Add(toCount,class);
		fi;
od;

return Sum(List(toCount,x->Size(x)));
end;

Test_1:=function(K)
	if NumberSubgroupsOrder_p(K) > 4 then
		return false;
	fi;
return true;
end;

Test_2:=function(K)
  local Z_K, p, bound, candidates, Z;

Z_K:=Center(K);
p:=PrimePGroup(K);

if p > 2 then bound:=0; else bound:=1; fi;

candidates:=Filtered(AllSubgroups(Z_K),x->Order(x)=p);

for Z in candidates do
	if NumberSubgroupsNotContainingCentralSubgroup(K,Z) <= bound then
		return true;
	fi;
od;

return false;

end;

Test_3:=function(K)
  local p;

p:=PrimePGroup(K);
	if Order(K) < p^3 then return false; fi;
#
	if CD_measure(K,K) <> Max_CD_measure(K) then return false; fi;

### to get here we have $|K| >= p^3$ and $K \in CD(K)$
	if NumberSubgroupsContainingCenterOutsideCDL(K) > 1 then return false; fi;

return true;

end;

ComputeDeltaCD:=function(G)

local SubgroupClasses, CD_LatticeClasses;

SubgroupClasses:=ConjugacyClassesSubgroups(G);
CD_LatticeClasses:=Filtered(
SubgroupClasses,x->CD_measure(G,Representative(x))=Max_CD_measure(G));

return Sum(List(SubgroupClasses,Size)) - Sum(List(CD_LatticeClasses,Size));
end;

TestSubgroupsOfOrderN:=function(n)
  local match;
Print(" ----------------- Test Results -----------------\n\n");
	for match in List(Filtered(AllSmallGroups(n),x-> Test_1(x) and Test_2(x) and Test_3(x)),IdSmallGroup) do
		Print(StringFormatted("SmallGroup({},{}) which is isomorphic to {} passes the tests\n\n",n,match[2],StructureDescription(SmallGroup(n,match[2]))));
		# Print(StringFormatted("{} passes the tests\n",));
	od;
end;

TestSubgroupsOfOrderN(32);

TestSubgroupsOfOrderN(243);


\end{verbatim}

\section*{Appendix B}
\textsc{MAGMA} code used to prove Lemma \ref{lem: 32} and Theorem \ref{thm: lt53}.

\input{cocke_code/check_conds1_2}


==> lt5_original.tex <==


\section{Proof of Theorem \ref{thm: lt5}}\label{sec: lt5}
Our proof of Theorem \ref{thm: lt5} is largely broken up into two parts: assume the group $G$ is abelian and classify; assume the group $G$ is not abelian and derive a contradiction. 

\begin{proposition}
If $G$ is a nonabelian finite group such that $\delta_{ \CD }(G) = 3$ then $G$ is a $2$-group such that:
\begin{itemize}
	\item $G$ has precisely $3$ involutions, only one of which is central.
	\item $\CD(G) = L(G) \cup {H_0,H_1,H_2}$ where $H_0$ is the trivial subgroup and $H_1,H_2$ are the two noncentral involutions.
	\item $|Z(G)| = 2$
	\item $|Im(m_G)|=2$  
	\item $\CD(G) = [G/Z(G)]$
	\item $|G|\geq 2^m$ where $m \geq 8$
\end{itemize}
\end{proposition}

\begin{proof}
Let $G$ be a nonabelian finite group of order $|G|=p^n$ such that $\delta_{ \CD }(G) = 3$. Then there exist three subgroups $H_0,H_1,H_2$ so that $\CD(G) = L(G) \cup \{ H_0,H_1,H_2 \} $ as $G$ is nilpotent it follows that $m_G(1) < m_G(Z(G))$ and it follows that one of these subgroups say $H_0$ is trivial.

Suppose $p,q,r$ are distinct primes dividing the order of $G$, then there exist Sylow subgroups $P \in Syl_p(G)$, $Q \in Syl_q(G)$ and $R \in Syl_r(G)$ such that $Z(P)$, $Z(Q)$ and $Z(R)$ all lie outside of $\CD(G)$ a contradiction. 

Suppose that $p$ and $q$ are distinct primes dividing the order of $G$ and $P \in Syl_p(G)$ and $Q \in Syl_q(G)$, since $m_G(1),m_G(Z(P)),m_G(Z(Q))$ and $m_G(Z(G))$ are distinct it must be the case that $|Im(m_G)|=4$. Since $m_G(G) \neq m_G(1)$ then by Theorem 2.1 of (cite Tarnauceanu 2020) this implies that $m_G(G) = m_G(H)$ where $H$ is a central subgroup of $Q$ or $P$, in either case this is a contradiction.


It follows that $G$ has at most one prime divisor. Now the Chermak-Delgado lattices for groups with a unique subgroup of order $p$ were classified in (cite Tarnauceanu2020) from which it follows that $G$ does not have a unique subgroup of order $p$, and in fact has at least 3, since the number of subgroups of order $p$ in a finite group are $1\mod p$. Now any proper subgroup of the center lies outside of $\CD(G)$, since any abelian group with more than 2 generators has at least 3 proper subgroups it follows that $Z(G)$ cyclic. Hence, all the noncentral subgroups of order $p$ lie outside of $\CD(G)$, from which it follows that $H_1$ and $H_2$ are subgroups of order $p$, and since there are precisely $3$ subgroups of order $p$ it follows that $p = 2$. As any proper subgroup of the center will lie outside of $\CD(G)$ it follows that $Z(G)$ is cyclic of order 2. Since $G \in \CD(G)$ it follows that $Im(m_G)=\{2^n,2^{ n+1 }\}$. 

That $\CD(G) = [G/Z(G]$ follows from Proposition 3.1 of (cite Tarnauceanu 2020 ). A direct computation of all $2$ groups dividing $2^7$ with $\delta_{\CD}(G)=3$ shows that $|G| > 2^7$.
\end{proof}


\begin{proposition}
If $G$ is a finite group and $\delta_{ \CD }(G) = 3$ then $G$ is abelian.
\end{proposition}

\begin{proof}
	Suppose that $G$ is non-abelian and $\Delta_{ \CD }(G) = 3$ then $G$ is a $2$-group of order $2^m$ where $m \geq 8$. Then there exist two non-central involutions $H_1,H_2$ and the trivial subgroup $H_0$ so that $\CD(G) = L(G) \cup \{ H_0,H_1,H_2 \}$. 

	First observe that there does not exist an abelian subgroup $A < G$ such that $|G:A|<4$. Suppose otherwise, then $|A| > 2$ and $A \in \CD(G)$. Since $|G:A| < 4$ it follows that $|A|\geq 2^{ m-2 }$, since $A \in \CD(G)$ and we know that $m(A)=2^{ m+1 }$, which implies that $|C_G(A)| = 2^3$ a contradiction since $A \subseteq C_G(A)$. From this it follows that $G$ is not of maximal class. 

	Let $B$ be a maximal normal non-cyclic abelian subgroup of $G$ of exponent at most $4$. Since $G$ is not of maximal class, $B$ is abelian of type $(4,2)$ or $(4,4)$. In either case by Corollary 10.2 (cite Berkovich2016 Groups of prime power order Vol 1) we have that $\Omega_2(C_G(B)) = B$. 

	Suppose that $B \cong C_4 \times C_2$, then $|\Omega_2(C_G(A))| = 8$ and by Lemma 42.1 (cite Berkovich2016 Groups of prime power order Vol 1) it follows that $C_G(A)$ is abelian of type $(2^n,2)$, $n \geq 2$. Since $A \in \CD(G)$ it follows that $C_G(A) \subset C_G(C_G(A))=A$, so that $A$ is self centralizing but this implies that the order of $G$ is $2^5$ a contradiction. So it must be the case that $B \cong C_4 \times C_4$, then $\Omega_1(B)$ is a normal $4$ subgroup of $G$. Let $B'$ be a normal subgroup of $G$ such that $\Omega_1(B) \leq B' \leq B$, then $B'$ is abelian of type $(4,2)$ and as before we have that $C_G(B')=B'$, which again yields a contradiction on the order of $G$. It follows that $G$ must be abelian.
\end{proof}



\begin{theorem}
	If $G$ is a finite group then $\delta_{\CD}(G) = 3$ if and only if $G \cong C_{ p^3 }$ or $G\cong C_p \times C_q$ for distinct primes $p$ and $q$.
\end{theorem}

\begin{proof}
	Suppose $G$ is a finite group with $\delta_{ CD }(G)=3$ from the previous proposition we know that $G$ is abelian. Then we have $\CD(G) = \{  G \} $, so if $\delta_{ \CD }(G) = 3$ it follows that $G$ has precisely 2 proper subgroups. Let $\pi(G)$ be the distinct prime divisors of $G$. If $|\pi(G)| \geq 3$, then there are at least $3$ proper nontrivial normal subgroups, so it must be the case that $|\pi(G)|<2$.

	Suppose $\pi(G) = \{ p,q \} $ where $p$ and $q$ are distinct primes, let $P \in Syl_p(G)$ and $Q \in Syl_q(G)$, which necessarily lie outside of $\CD(G)$ and are simple, it follows that $G \cong P \times Q$ and $|G|=pq$.

	Suppose $ \pi(G) = \{ p \}  $. Observe that if $G$ has more than one generator, then $G$ has at least $3$ proper nontrivial subgroups, it follows that $G$ is cyclic and has precisely 2 nontrivial proper subgroups from which it follows that $G \cong C_{ p^3 }$ and $|G|=p^3$.
\end{proof}


==> previous_versions/alternative_proofs.tex <==

\section{Proof of Theorem \ref{thm: lt5}}


\begin{lemma}\label{lem: lt5->p-group}
Let $G$ be a nonabelian nilpotent group. If $\delta_{\CD}(G) < 7,$ then $G$ is a $p$-group. If $\delta_{\CD}{G} < 6$, then $G$ is a $2$-group or a $3$-group.
\end{lemma}

\begin{proof}
Suppose that $G$ is not a $p$-group, i.e., there are at least two prime divisors of $G$. Lemma \ref{cor: no_p_groups_nil} tells us that no $p$-groups are in $\CD(G)$. Moreover, since $G$ is nonabelian, then at least one Sylow subgroup $S$ of $G$ is nonabelian. Nonabelian $p$-groups have at least $p+2$ subgroups above the center, which means they have at least $p+4$ subgroups total. Thus $G$ contains $p+4$ distinct $p$-groups for the prime $p$.

Together with a nontrivial Sylow $q$-group $T$, these form a set of $p+5$ subgroups that witness $\delta_{\CD(G)}\geq p+5$. 

Thus we have \[p+5 \leq \delta_{\CD}(G) < 7,\] and we conclude that $G$ must be a $p$-group. 

Recall that a nonabelian $p$-group of odd order must contain $p+1$ subgroups of order $p$. By Lemma \ref{lem: order_p_witnesses} this means that 
\[p+1 \leq \delta_{\CD}(G) <6\] and we conclude that $p<4.$
 
\end{proof}

We note that for an odd prime $\delta_{\CD}(Q_8 \times C_p) = 7$ and is a nonabelian nilpotent group, so the bound given in Lemma \ref{lem: lt5->p-group} is sharp.  


\begin{lemma}\label{lem: lt5_conds}
Let $G$ be a nonabelian $p$-group and suppose $3\leq \delta_{\CD(G)} \leq 4$. For any $K\leq G$ the following hold:
\begin{enumerate}
    \item There are at most $4$ subgroups of order $p$ in $K$.
    \item There is a subgroup $Z\leq \mathbf{Z}(K)$ with $|Z|=p$ such that \[|\{H\leq K: p^2\leq |K|\text{ and } Z\not < K\}| \leq 1.\]
    \item At most one subgroup of $K$ can violate the following: \[|\{H \leq K: p^2\leq |H| \text{ and } \CD(H) \neq [[Z(H):H]]\} | \leq 1.\]
\end{enumerate}
\end{lemma}

\begin{proof}
1. If $K$ had more than 4 subgroups, then it would have at least $5$ such groups. Hence $G$ would have at least 5 subgroups of order $p$ and by Lemma \ref{lem: order_p_witnesses} $\delta_{\CD}(G) \geq 5$. 

2.  If $K$ has a single single subgroup of order $p$ it is cyclic and trivially satisfies the hypothesis. 

By Lemma \ref{lem: lt5->p-group}, we know that $p$ is either 2 or 3.  
Suppose that $p=2$. Then $K$ contains three subgroups $A=\langle a \rangle $, $B=\langle b\rangle$, and $C=\langle ab\rangle$ of order 2. If none of them are in $\CD(G)$, then the four subgroups not in $\CD(G)$ are $\{1, A,B,C\}$  Then $\CD(G)$ contains $AB=\langle a, b\rangle$ and $AB \leq \textbf{Z}(G)$. Moreover, since $\delta_{\CD(G)} = 4$ in this case, we conclude that every subgroup of $G$ of order $4$ or larger is contained in $\CD(G)$, and thus contains $\textbf{Z}(G) = \langle a,b\rangle$.
Otherwise let $Z\leq H$ of order 2 in $\CD(G)$. Since $Z\in \CD(G)$, we know that $Z=\mathbf{Z}(G)$ and hence $Z\leq \mathbf{Z}(K)$. Moreover, since the other two involutions and the identity would not be in $\CD(G)$, we have $\delta_{\CD(G)} \geq 3$ and thus at most one other subgroup of $G$ (which must have order greater than 2) could not be in $\CD(G)$ and thus not contain $Z$. 

Suppose that $p=3$. Then $K$ contains four subgroups $A,B,C$ and $D$ of order $3$. Since $\delta_{\CD}(G) = 4$. We note that exactly one of these subgroups say $A$ is contained in $\CD(G)$. Then every subgroup of $G$ except for $1,B,C,D$ is contained in $\CD(G)$ and must contain $A$ as a subgroup. 

3. Any subgroup in $\CD(G)$ must satisfy $\CD(H) = [[Z(H):H]]$. There is at most one subgroup of order $p^2$ not contained in $\CD(G)$. Hence $K$ can have at most one such subgroup. 
\end{proof}

Lemma \ref{lem: lt5_conds} gives us conditions on the types of subgroups a $2$-group or $3$-group $G$ can have if $3\leq \delta_{\CD(G)} \leq 4$. This allows us to specify what types of subgroups $G$ can have of a given order. For example, a $2$-group $G$ with $3\leq \delta_{\CD(G)} \leq 4$ cannot contain the dihedral group of order $8$ as a subgroup because the dihedral group of order $8$ has 5 involutions. Similarly, it cannot contain the elementary abelian group of order $8$ as a subgroup. This means all of its subgroups of order $8$ are either cyclic, quaternion, or isomorphic to $C_4\times C_2$. We can computationally then search over all of the $2$-groups of a given order to look for potential subgroups of a group 2-group $G$ with $3\leq \delta_{\CD(G)} \leq 4.$ 

We will pause to introduce the reader to another family of $p$-groups. These groups are commonly written as $M_{p^k} = \langle a, b | a^{p^{k-1}},b^{p}, a^b= a^{p^{k-2}+1}\rangle.$ For an odd prime $p$, the groups $M_{p^k}$ are the only nonabelian $p$-groups with cyclic maximal subgroups. This fact is 

\begin{lemma}
Let $G$ be a $2$-group and suppose $3\leq \delta_{\CD(G)} \leq 4$. Then

\begin{enumerate}
    \item All subgroups of order $8$ in $G$ are either cyclic, quaternion, or isomorphic to $C_4\times C_2$. 
    \item All subgroups of order $16$ in $G$ are isomorphic to one of the following groups: $C_{16},\, C_8 \times C_2,\, M_{16},\,$ or $ Q_8 \times C_2$.  
    \item All subgroups of order $32$ in $G$ are isomorphic to one of the following groups: $C_{32},\, C_{16}\times C_2,\,$ or $ M_{32}$. 
\end{enumerate}
\end{lemma}
\begin{proof}
 
\end{proof}

We could continue our calculations and would see that there are 3 possible subgroups of order 64 which are $C_{64}, C_{32} \times C_2$ and $M_{64}$. Similarly, we would see that there are 3 possible subgroups of order 128, i.e., the groups $C_{128}, C_{64}\times C_2, M_{128}.$ There are also 3 possible subgroups of order 256. This observation motivates the following theorem. 


\begin{theorem}\label{thm: up}
Let $G$ be a $p$-group with order $|G| = p^{k+1} \geq 32$. Suppose that $G$ contains only p+1 subgroups of order $p$ and that the only maximal subgroups of $G$ are isomorphic to $C_{p^k}, C_{p^{k-1}}\times C_p$, and $M_{p^k}$. Then $G$ is isomorphic to one of the groups $C_{p^k+1}, C_{p^{k-1}} \times C_p$, or $M_{p^{k+1}}$.
\end{theorem}

\begin{proof}
If $G$ is abelian, then it must be isomorphic to either $C_{p^k}$ or $C_{p^{k-1}} \times C_p$. 

If not abelian, then if all maximal subgroups are abelian, we have that $G$ is $M_{p^k}$. 

Now suppose that $G$ has a maximal nonabelian subgroup $M$, i.e., $M\cong M_{p^k}$. We note that $G$ has another maximal subgroup $K$. Suppose that $K$ is isomorphic to $C_{p^{k-1}} \times C_p$. Then, there are distinct subgroups $A$,$B$ of order $p$ in $G$ that commute and subgroups $C$,$D$ of order $p$ in $G$ that do not commute. Hence there are more than $p+1$ subgroups of order $p$. 

If $K$ is isomorphic to $C_{p^{k}}$, then identify $a,b\in M$ such that $M=\langle a, b | a^{p^{k-1}},b^p, a^b = a^{p^{k-2}+1}\rangle$. We note that $b\notin K$ since otherwise there would be too many elements of order $p$. It must be the case that $[K,b] \neq 1$. Hence, $K^b = K$. We conclue that $a\in K$. If $K=\langle c \rangle$, then $c^b$ must satisfy $(c^b)^p = a^b.$ This is implies that $b$ acts fixed point free on $K/p^{k-2} \cong C_{p^2}$. There are no such actions. 

Suppose now that $K$ is isomorphic to $M$. If the subgroups of order $p^{k-1}$ are not the same, then we have too many elements of order $p$. If the subgroups are the same, then there are too many elements of order $p$ coming from the noncommutating pieces. 
\end{proof}

For $3$-groups, Lemma \ref{lem: lt5_conds} can be used to establish the following.

\begin{lemma}
Let $G$ be a nonabelian $3$-group with  $\delta_{\CD(G)} = 4$. Then \begin{enumerate}
    \item All subgroups of order $27$ in $G$ are isomorphic to one of $C_{27},\, C_{9}\times C_3,$ or $M_{27}$.
\end{enumerate} \end{lemma}

The reader should notice the wonderful fact that these are the same 3 types of groups that occur in Theorem \ref{thm: up}. This means that as in the 2-group case, for a $3$-group with $\delta_{\CD}(G) = 4$ there are at most three isomorphism classes of subgroups for any order greater than 27.

\begin{theorem}
If $G$ is a nonabelian $2$-group and $\delta_{\CD(G)} \leq 4$, then $G$ is the quaternion group of order $8$.
\end{theorem}

\begin{proof}
If $G$ has a single involution, then $G$ is quaternion and we note that $m_{\CD(G)} = \left(\frac{|G|}{2}\right)^2$. If $|G| > 8$, then $\CD(G)$ is a single subgroup and $\delta_{\CD(G)} > 4.$

Suppose by way of contradiction, that $G$ is not the quaternion group of order $8$. We must have that $3\leq \delta_{\CD(G)} \leq 4$. As noted, in Lemma \ref{lem: 32} the only subgroups of order $32$ in $G$ would be isomorphic to $C_{32}, C_{16}\times C_2$, or $M_{32}$. By Theorem \ref{thm: up}, the only subgroups of order 64 in $G$ would be isomorphic to $C_{64}, C_{32}\times C_2$ or $M_{64}$. Continuing in this manner, we see that eventually $G$ would be isomorphic to either $C_{2^k}, C_{2^{k-1}}\times C_{2}$ or $M_{2^k}$. However, none of these groups satisfy $\delta_{\CD(G)} \leq 4$. 

Thus $|G| \leq 32$. A computational search using $\textsc{MAGMA}$ shows there is no such nonabelian $2$-group. 
\end{proof}

\begin{theorem}
If $G$ is a nonabelian $3$-group, then $\delta_{\CD(G)} \geq 5$.
\end{theorem}

\begin{proof}
We note that all of the subgroups of $G$ of order 27 would be isomorphic to $C_{27}, C_9 \times C_2$, or $M_{27}$. By Theorem $\ref{thm: up}$, $G$ itself is isomorphic to $C_{3^k}, C_{3^{k-1}}\times C_3,$ or $M_{3^k}$. These groups do not satisfy $\delta_{\CD(G)} \leq 4$. 
\end{proof}


==> previous_versions/lt5_original.tex <==


\section{Proof of Theorem \ref{thm: lt5}}\label{sec: lt5}
Our proof of Theorem \ref{thm: lt5} is largely broken up into two parts: assume the group $G$ is abelian and classify; assume the group $G$ is not abelian and derive a contradiction. 

\begin{proposition}
If $G$ is a nonabelian finite group such that $\delta_{ \CD }(G) = 3$ then $G$ is a $2$-group such that:
\begin{itemize}
	\item $G$ has precisely $3$ involutions, only one of which is central.
	\item $\CD(G) = L(G) \cup {H_0,H_1,H_2}$ where $H_0$ is the trivial subgroup and $H_1,H_2$ are the two noncentral involutions.
	\item $|Z(G)| = 2$
	\item $|Im(m_G)|=2$  
	\item $\CD(G) = [G/Z(G)]$
	\item $|G|\geq 2^m$ where $m \geq 8$
\end{itemize}
\end{proposition}

\begin{proof}
Let $G$ be a nonabelian finite group of order $|G|=p^n$ such that $\delta_{ \CD }(G) = 3$. Then there exist three subgroups $H_0,H_1,H_2$ so that $\CD(G) = L(G) \cup \{ H_0,H_1,H_2 \} $ as $G$ is nilpotent it follows that $m_G(1) < m_G(Z(G))$ and it follows that one of these subgroups say $H_0$ is trivial.

Suppose $p,q,r$ are distinct primes dividing the order of $G$, then there exist Sylow subgroups $P \in Syl_p(G)$, $Q \in Syl_q(G)$ and $R \in Syl_r(G)$ such that $Z(P)$, $Z(Q)$ and $Z(R)$ all lie outside of $\CD(G)$ a contradiction. 

Suppose that $p$ and $q$ are distinct primes dividing the order of $G$ and $P \in Syl_p(G)$ and $Q \in Syl_q(G)$, since $m_G(1),m_G(Z(P)),m_G(Z(Q))$ and $m_G(Z(G))$ are distinct it must be the case that $|Im(m_G)|=4$. Since $m_G(G) \neq m_G(1)$ then by Theorem 2.1 of (cite Tarnauceanu 2020) this implies that $m_G(G) = m_G(H)$ where $H$ is a central subgroup of $Q$ or $P$, in either case this is a contradiction.


It follows that $G$ has at most one prime divisor. Now the Chermak-Delgado lattices for groups with a unique subgroup of order $p$ were classified in (cite Tarnauceanu2020) from which it follows that $G$ does not have a unique subgroup of order $p$, and in fact has at least 3, since the number of subgroups of order $p$ in a finite group are $1\mod p$. Now any proper subgroup of the center lies outside of $\CD(G)$, since any abelian group with more than 2 generators has at least 3 proper subgroups it follows that $Z(G)$ cyclic. Hence, all the noncentral subgroups of order $p$ lie outside of $\CD(G)$, from which it follows that $H_1$ and $H_2$ are subgroups of order $p$, and since there are precisely $3$ subgroups of order $p$ it follows that $p = 2$. As any proper subgroup of the center will lie outside of $\CD(G)$ it follows that $Z(G)$ is cyclic of order 2. Since $G \in \CD(G)$ it follows that $Im(m_G)=\{2^n,2^{ n+1 }\}$. 

That $\CD(G) = [G/Z(G]$ follows from Proposition 3.1 of (cite Tarnauceanu 2020 ). A direct computation of all $2$ groups dividing $2^7$ with $\delta_{\CD}(G)=3$ shows that $|G| > 2^7$.
\end{proof}


\begin{proposition}
If $G$ is a finite group and $\delta_{ \CD }(G) = 3$ then $G$ is abelian.
\end{proposition}

\begin{proof}
	Suppose that $G$ is non-abelian and $\Delta_{ \CD }(G) = 3$ then $G$ is a $2$-group of order $2^m$ where $m \geq 8$. Then there exist two non-central involutions $H_1,H_2$ and the trivial subgroup $H_0$ so that $\CD(G) = L(G) \cup \{ H_0,H_1,H_2 \}$. 

	First observe that there does not exist an abelian subgroup $A < G$ such that $|G:A|<4$. Suppose otherwise, then $|A| > 2$ and $A \in \CD(G)$. Since $|G:A| < 4$ it follows that $|A|\geq 2^{ m-2 }$, since $A \in \CD(G)$ and we know that $m(A)=2^{ m+1 }$, which implies that $|C_G(A)| = 2^3$ a contradiction since $A \subseteq C_G(A)$. From this it follows that $G$ is not of maximal class. 

	Let $B$ be a maximal normal non-cyclic abelian subgroup of $G$ of exponent at most $4$. Since $G$ is not of maximal class, $B$ is abelian of type $(4,2)$ or $(4,4)$. In either case by Corollary 10.2 (cite Berkovich2016 Groups of prime power order Vol 1) we have that $\Omega_2(C_G(B)) = B$. 

	Suppose that $B \cong C_4 \times C_2$, then $|\Omega_2(C_G(A))| = 8$ and by Lemma 42.1 (cite Berkovich2016 Groups of prime power order Vol 1) it follows that $C_G(A)$ is abelian of type $(2^n,2)$, $n \geq 2$. Since $A \in \CD(G)$ it follows that $C_G(A) \subset C_G(C_G(A))=A$, so that $A$ is self centralizing but this implies that the order of $G$ is $2^5$ a contradiction. So it must be the case that $B \cong C_4 \times C_4$, then $\Omega_1(B)$ is a normal $4$ subgroup of $G$. Let $B'$ be a normal subgroup of $G$ such that $\Omega_1(B) \leq B' \leq B$, then $B'$ is abelian of type $(4,2)$ and as before we have that $C_G(B')=B'$, which again yields a contradiction on the order of $G$. It follows that $G$ must be abelian.
\end{proof}



\begin{theorem}
	If $G$ is a finite group then $\delta_{\CD}(G) = 3$ if and only if $G \cong C_{ p^3 }$ or $G\cong C_p \times C_q$ for distinct primes $p$ and $q$.
\end{theorem}

\begin{proof}
	Suppose $G$ is a finite group with $\delta_{ CD }(G)=3$ from the previous proposition we know that $G$ is abelian. Then we have $\CD(G) = \{  G \} $, so if $\delta_{ \CD }(G) = 3$ it follows that $G$ has precisely 2 proper subgroups. Let $\pi(G)$ be the distinct prime divisors of $G$. If $|\pi(G)| \geq 3$, then there are at least $3$ proper nontrivial normal subgroups, so it must be the case that $|\pi(G)|<2$.

	Suppose $\pi(G) = \{ p,q \} $ where $p$ and $q$ are distinct primes, let $P \in Syl_p(G)$ and $Q \in Syl_q(G)$, which necessarily lie outside of $\CD(G)$ and are simple, it follows that $G \cong P \times Q$ and $|G|=pq$.

	Suppose $ \pi(G) = \{ p \}  $. Observe that if $G$ has more than one generator, then $G$ has at least $3$ proper nontrivial subgroups, it follows that $G$ is cyclic and has precisely 2 nontrivial proper subgroups from which it follows that $G \cong C_{ p^3 }$ and $|G|=p^3$.
\end{proof}


==> previous_versions/open_questions.tex <==

\section{Open Questions} \label{sec:opn}
If a group is divisible by $k$ primes counting with multiplicity, is $\delta_{\CD(G)} \geq k-2$? 


==> previous_versions/s3_alternative.tex <==

\section{Proof of Theorem \ref{thm: s3}.}

If a finite group $G$ is not nilpotent, then it has at least $4$ Sylow subgroups, and if $G$ has either four or five Sylow subgroups, then $G$ is a $\{2,3\}$-group. In this section we will sometimes use the non-standard notation $H_p$ to denote a Sylow $p$-subgroup of $G$. This is to make our proofs easier to read by reminding the reader of the prime associated with the Sylow $p$-subgroup, especially as the prime $p$ will shift between certain lemmata. In addition, we wish to avoid confusion with $S_p$, the symmetric group on $p$-symbols. 

\begin{lemma}\label{lem: 1_2_4_3}
Suppose that a finite $\{2,3\}$-group $G$ has exactly four Sylow $3$-subgroups and a normal $2$-subgroup $H_2$. Then $\delta_{\CD}(G) > 5$.
\end{lemma}

\begin{proof}
Since $G$ has four Sylow $3$-subgroups, it is not nilpotent. By Theorem \ref{thm: nil}, we conclude that $\delta_{\CD}(G) \geq 5$.
The four Sylow $3$-subgroups of $G$ witness that $\delta_{\CD}(G) \geq 4$. By way of contradiction suppose that $\delta_{\CD}(G) = 5$.  

Suppose $1\in \CD(G)$. By Lemma \ref{lem: no_p_groups}, no nontrivial $p$-groups of any order are in $\CD(G)$ for any prime $p$. Hence $G$ has exactly five total nontrivial $2$-groups or $3$-groups, namely the four Sylow $3$-groups and the normal Sylow $2$-group.  We conclude that all of the nontrivial Sylow subgroups have prime order, and $|G|=6$. But then a Sylow $3$-group has Chermak-Delgado measure of $9$ which is larger than $m^*(G) = 6$, a contradiction.

Now suppose that $1\notin \CD(G)$. By assumption, $1$ and the four Sylow $3$-subgroups are the only subgroups of $G$ not contained in $\CD(G)$. Hence $G$ and $H_2$ are in $\CD(G)$. This means that $m^*(G) = |G| \cdot |\textbf{Z}(G)|$ is divisible by $|G|$. But, $m^{*}(G) = |H_2|\cdot |\textbf{C}_G(H_2)|$. Since $H_2$ is a $2$-group, we conclude that $[H_2,T]=1$ for a Sylow $3$-subgroup $T$ of $G$. Then $H_2T =G$ is a direct product and is thus nilpotent, a contradiction. Hence $\delta_{\CD}(G) > 5.$
\end{proof}

\begin{lemma}\label{lem:3_2_1_3}
Suppose that a finite $\{2,3\}$-group $G$ has exactly three Sylow $2$-subgroups and a normal Sylow $3$-subgroup $H_3$. If $\delta_{\CD}(G) = 5$, then $1\notin \CD(G)$.
\end{lemma}
\begin{proof}
Suppose by way of contradiction that $1\in \CD(G)$. By Lemma \ref{lem: no_p_groups} no nontrivial $p$-groups of any order are in $\CD(G)$ for any prime $p$. Hence $G$ has at most five nontrivial $2$-groups or $3$-groups, including the three Sylow $2$-subgroups and $H_3$.  And so $G$ has at most two subgroups that are nontrivial $3$-groups, and at most one subgroup that is a nontrivial $2$-group, but not Sylow.  This means that $G$ is a $\{2,3\}$-group with $|G| \leq 2^2 3^2$.  Considering each of the possible orders of $G$, $2 \cdot 3$, $4 \cdot 3$, $2 \cdot 9$, or $4 \cdot 9$, we see that in each case, a Sylow subgroup of $G$ has Chermak--Delgado measure larger than $m^*(G) = |G|$.
\end{proof}

\begin{lemma}\label{lem: H_3inCD}
Suppose that a finite $\{2,3\}$-group $G$ has exactly three Sylow $2$-subgroups and a normal Sylow $3$-subgroup $H_3$. If $\delta_{\CD}(G) = 5$, then $H_3 \in \CD(G)$.\end{lemma}
\begin{proof}
By Lemma \ref{lem:3_2_1_3}, we know that $1\notin \CD(G)$. Hence $1$, together with the three Sylow $2$-subgroups witness that $\delta_{\CD}(G) \geq 4$. There is one other subgroup of $G$ not contained in $\CD(G)$. 

Suppose by way of contradiction that $H_3 \notin \CD(G)$. Let $T_2$ be a Sylow $2$-subgroup.  We claim that one of $H_3$ or $T_2$ must have prime order. Otherwise, if $1 < P < H_3$, and $1 < Q < T_2$, then $P,Q \in \CD(G)$, and so $1 = P \cap Q \in \CD(G)$, a contradiction. Let $K$ be a Sylow subgroup of prime order $p$. %Without loss of generality, suppose $T$ has prime order.  (The argument for $S$ would be similar.)

Then $K \cap \textbf{Z}(G) = 1$, as otherwise, $K \leq \textbf{Z}(G)$, and it would follow that the $\{2,3\}$-group $G$ is nilpotent. And so $\textbf{Z}(G)$ is a $p'$-group.  Now $m^*(G) = |G||\textbf{Z}(G)| = p \cdot (p')^i$ for some $i$.  But also $K < K\textbf{Z}(G) < G$, and so $K\textbf{Z}(G) \in \CD(G)$.  But $K\textbf{Z}(G)$ is abelian, and so $K\textbf{Z}(G) \leq \textbf{C}_G(K\textbf{Z}(G))$, and so $p^2$ divides $|K\textbf{Z}(G)||\textbf{C}_G(K\textbf{Z}(G))| = m^*(G)$, a contradiction.

\end{proof}

We can now prove Theorem \ref{thm: s3}, which states that for a non-nilpotent group we have $\delta_{\CD}(G) = 5 \rightarrow G \cong S_3$. 

\begin{proof}[Proof of Theorem \ref{thm: s3}.]
From Lemma \ref{lem: 1_2_4_3} we conclude that $G$ is a $\{2,3\}$ group with exactly three Sylow $2$-subgroups, and a normal Sylow $3$-subgroup $H_3$. From Lemmata \ref{lem:3_2_1_3} and \ref{lem: H_3inCD} we have that the five subgroups of $G$ not contained in $\CD(G)$ are the three Sylow $2$-subgroups, the identity subgroup, and one other subgroup $X$. We will show that $X=G$. Suppose instead that $G\in \CD(G)$. 

Note that any Sylow $2$-subgroup of $\textbf{C}_G(H_3)$ is also a Sylow $2$-subgroup of $G$.  This is because $|H_3||\textbf{C}_G(H_3)| = m^*(G)$ and since $G \in \CD(G)$, $|G|$ divides $m^*(G)$.  And so now we have that $G=H_3 T$ is a direct product where $T$ is a Sylow $2$-subgroup of $\textbf{C}_G(H_3)$, which implies that $G$ is nilpotent, a contradiction.

So $X=G$, and the three Sylow $2$-subgroups, the identity subgroup, and $G$ witness that $\delta_{\CD}(G) = 5.$

Let $T$ be a Sylow $2$-subgroup of $G$.  We argue that $|T|=2$.  Otherwise, there exists $1 < X \leq \textbf{Z}(T)$ with $X < T$, and so $X \in \CD(G)$. Then $m^*(G) = |X||\textbf{C}_G(X)| = |H_3||\textbf{C}_G(H_3)|$, and so $|H_3|$ divides $|\textbf{C}_G(X)|$. This implies that $H_3 \leq \textbf{C}_G(X)$. Hence $[X,T]=1$ and $[X,H_3]=1$. Since $\textbf{Z}(G) \leq H_3$, we have $X \leq \textbf{Z}(G) \leq H_3$, a contradiction. Hence $|T|=2$.  Since $|T|=2$, we note that $\textbf{C}_G(H_3)$ is a $3$-group as otherwise a Sylow $2$-subgroup would be contained in $\textbf{C}_G(H_3)$ which would imply that $G$ is nilpotent.  So $m^*(G) = |H_3||\textbf{C}_G(H_3)|$ is a power of $3$.  

We now argue that $T$ is self-normalizing.  Suppose that $Y$ is a nontrivial Sylow $3$-subgroup of $\textbf{N}_G(T)$.  So $1 < Y < S$ (note that $Y < S$ as otherwise $S$ and $T$ would normalize one another, and so $G=ST$ would be nilpotent).  Then $TY$ is a subgroup, and $T < TY < G$, and so $TY$ is in $\CD(G)$, which contradicts the fact that $m^*(G)$ is a power of $3$.

So $T$ is self-normalizing, and $3 = |G:\textbf{N}_G(T)| = |G:T| = |H_3|$.  So $H_3$ is cyclic of order $3$, $T$ is cyclic of order $2$, and $G = S_3$ with $\CD(G) = \{ H_3\}$.
\end{proof}

==> previous_versions/s3_original.tex <==

\begin{proposition}\label{prop:delta_5_non_nilp}
Suppose $G$ is a finite group and $G$ is not nilpotent and suppose $\delta_{ \CD }(G) = 5$.  Then $G = S_3$. 
\end{proposition}

\begin{proof}
Case 1: $G$ has four Sylow $3$-subgroups and a normal Sylow $2$-subgroup, say $S$.  First suppose $S \notin \CD(G)$.  Then $1 \in \CD(G)$, and it follows by Lemma \ref{lem: no_p_groups} that the Sylow subgroups of $G$ all have prime order.  But then $4$ divides $2$, a contradiction.  So $S \in \CD(G)$, and so the four Sylow $3$-subgroups and the identity subgroup are the subgroups that are not in $\CD(G)$.  And so $G \in \CD(G)$.  

Note that any Sylow $3$-subgroup of $\textbf{C}_G(S)$ is also a Sylow $3$-subgroup of $G$.  This is because $|S||\textbf{C}_G(S)| = m^*(G)$ and since $G \in \CD(G)$, $|G|$ divides $m^*(G)$.  And so now we have that $G=ST$ is a direct product where $T$ is a Sylow $3$-subgroup of $\textbf{C}_G(S)$, which implies that $G$ is nilpotent, a contradiction.

Case 2: $G$ has three Sylow $2$-subgroups and a normal Sylow $3$-subgroup, say $S$.  First suppose $S \notin \CD(G)$.  And so the five subgroups not in $\CD(G)$ are the three Sylow $2$-subgroups, $S$, and one other subgroup $X$.  If $X \neq 1$, then $1 \in \CD(G)$, and it follows by Lemma \ref{lem: no_p_groups} that the Sylow subgroups of $G$ all have prime order.  And so $6 = |G| = m^*(G)$, but $m_G(S) = 9$, a contradiction.  So $X=1$, and so $G \in \CD(G)$ and $\textbf{Z}(G) > 1$. 

Now the five subgroups not in $\CD(G)$ are the three Sylow $2$-subgroups, $S$, and the identity subgroup.  Let $T$ be a Sylow $2$-subgroup.  Note that one of $S$ or $T$ must have prime order.  This is because, otherwise, if $1 < P < S$, and $1 < Q < T$, then $P,Q \in \CD(G)$, and so $1 < \textbf{Z}(G) \leq P \cap Q$, a contradiction (note that $P$ and $Q$ contain $\textbf{Z}(G)$ since they are both in $\CD(G)$). Without loss of generality, suppose $T$ has prime order.  (The argument for $S$ would be similar.)

And so $T \cap \textbf{Z}(G) = 1$, as otherwise, $T \leq \textbf{Z}(G)$, and it would follow that $G = ST$ is nilpotent. And so $\textbf{Z}(G)$ is a $3$-group.  Now $m^*(G) = |G||\textbf{Z}(G)| = 2 \cdot 3^i$ for some $i$.  But also $T < T\textbf{Z}(G) < G$, and so $T\textbf{Z}(G) \in \CD(G)$.  But $T\textbf{Z}(G)$ is abelian, and so $T\textbf{Z}(G) \leq \textbf{C}_G(T\textbf{Z}(G))$, and so $4$ divides $|T\textbf{Z}(G)||\textbf{C}_G(T\textbf{Z}(G))| = m^*(G)$, a contradiction.

And so $S \in \CD(G)$, and so $1 \notin \CD(G)$.  And so the five subgroups not in $\CD(G)$ are the three Sylow $2$-subgroups, the identity subgroup, and one other subgroup $X$.  We argue that $X=G$.  Otherwise, $G \in \CD(G)$.

But, similar to before, note that any Sylow $2$-subgroup of $\textbf{C}_G(S)$ is also a Sylow $2$-subgroup of $G$.  This is because $|S||\textbf{C}_G(S)| = m^*(G)$ and since $G \in \CD(G)$, $|G|$ divides $m^*(G)$.  And so now we have that $G=ST$ is a direct product where $T$ is a Sylow $2$-subgroup of $\textbf{C}_G(S)$, which implies that $G$ is nilpotent, a contradiction.

So $X=G$, and the five subgroups not in $\CD(G)$ are the three Sylow $2$-subgroups, the identity subgroup, and $G$.

Let $T$ be a Sylow $2$-subgroup of $G$.  We argue that $|T|=2$.  Otherwise, there exists $1 < X \leq \textbf{Z}(T)$ with $X < T$, and so $X \in \CD(G)$.  Note that $m^*(G) = |X||\textbf{C}_G(X)| = |S||\textbf{C}_G(S)|$, and so $|S|$ divides $|\textbf{C}_G(X)|$.  And so $S \leq \textbf{C}_G(X)$ and so $X \leq \textbf{Z}(G) \leq S$, a contradiction (note $S$ contains $\textbf{Z}(G)$ since $S$ is in $\CD(G)$).

Hence $|T|=2$.  Note that $\textbf{C}_G(S)$ is a $3$-group as otherwise, since $|T|=2$, we would have a Sylow $2$-subgroup contained in $\textbf{C}_G(S)$, and hence $G$ is nilpotent, a contradiction.  And so $m^*(G) = |S||\textbf{C}_G(S)|$ is a power of $3$.  

Next, we argue that $T$ is self-normalizing.  Otherwise, let $Y$ be a Sylow $3$-subgroup of $\textbf{N}_G(T)$.  So $1 < Y < S$ (note that $Y < S$ as otherwise $S$ and $T$ would normalize one another, and so $G=ST$ would be nilpotent).  

But then $TY$ is a subgroup, and $T < TY < G$, and so $TY$ is in $\CD(G)$, which contradicts the fact that $m^*(G)$ is a power of $3$.

So $T$ is self-normalizing, and $3 = |G:\textbf{N}_G(T)| = |G:T| = |S|$.  So $S$ is cyclic of order $3$, $T$ is cyclic of order $2$, and $G = S_3$ with $\CD(G) = \{ S \}$ and, sure enough, $\delta_{ \CD }(G) = 5$.
\end{proof}

==> s3_original.tex <==

\begin{proposition}\label{prop:delta_5_non_nilp}
Suppose $G$ is a finite group and $G$ is not nilpotent and suppose $\delta_{ \CD }(G) = 5$.  Then $G = S_3$. 
\end{proposition}

\begin{proof}
Case 1: $G$ has four Sylow $3$-subgroups and a normal Sylow $2$-subgroup, say $S$.  First suppose $S \notin \CD(G)$.  Then $1 \in \CD(G)$, and it follows by Lemma \ref{lem: no_p_groups} that the Sylow subgroups of $G$ all have prime order.  But then $4$ divides $2$, a contradiction.  So $S \in \CD(G)$, and so the four Sylow $3$-subgroups and the identity subgroup are the subgroups that are not in $\CD(G)$.  And so $G \in \CD(G)$.  

Note that any Sylow $3$-subgroup of $\textbf{C}_G(S)$ is also a Sylow $3$-subgroup of $G$.  This is because $|S||\textbf{C}_G(S)| = m^*(G)$ and since $G \in \CD(G)$, $|G|$ divides $m^*(G)$.  And so now we have that $G=ST$ is a direct product where $T$ is a Sylow $3$-subgroup of $\textbf{C}_G(S)$, which implies that $G$ is nilpotent, a contradiction.

Case 2: $G$ has three Sylow $2$-subgroups and a normal Sylow $3$-subgroup, say $S$.  First suppose $S \notin \CD(G)$.  And so the five subgroups not in $\CD(G)$ are the three Sylow $2$-subgroups, $S$, and one other subgroup $X$.  If $X \neq 1$, then $1 \in \CD(G)$, and it follows by Lemma \ref{lem: no_p_groups} that the Sylow subgroups of $G$ all have prime order.  And so $6 = |G| = m^*(G)$, but $m_G(S) = 9$, a contradiction.  So $X=1$, and so $G \in \CD(G)$ and $\textbf{Z}(G) > 1$. 

Now the five subgroups not in $\CD(G)$ are the three Sylow $2$-subgroups, $S$, and the identity subgroup.  Let $T$ be a Sylow $2$-subgroup.  Note that one of $S$ or $T$ must have prime order.  This is because, otherwise, if $1 < P < S$, and $1 < Q < T$, then $P,Q \in \CD(G)$, and so $1 < \textbf{Z}(G) \leq P \cap Q$, a contradiction (note that $P$ and $Q$ contain $\textbf{Z}(G)$ since they are both in $\CD(G)$). Without loss of generality, suppose $T$ has prime order.  (The argument for $S$ would be similar.)

And so $T \cap \textbf{Z}(G) = 1$, as otherwise, $T \leq \textbf{Z}(G)$, and it would follow that $G = ST$ is nilpotent. And so $\textbf{Z}(G)$ is a $3$-group.  Now $m^*(G) = |G||\textbf{Z}(G)| = 2 \cdot 3^i$ for some $i$.  But also $T < T\textbf{Z}(G) < G$, and so $T\textbf{Z}(G) \in \CD(G)$.  But $T\textbf{Z}(G)$ is abelian, and so $T\textbf{Z}(G) \leq \textbf{C}_G(T\textbf{Z}(G))$, and so $4$ divides $|T\textbf{Z}(G)||\textbf{C}_G(T\textbf{Z}(G))| = m^*(G)$, a contradiction.

And so $S \in \CD(G)$, and so $1 \notin \CD(G)$.  And so the five subgroups not in $\CD(G)$ are the three Sylow $2$-subgroups, the identity subgroup, and one other subgroup $X$.  We argue that $X=G$.  Otherwise, $G \in \CD(G)$.

But, similar to before, note that any Sylow $2$-subgroup of $\textbf{C}_G(S)$ is also a Sylow $2$-subgroup of $G$.  This is because $|S||\textbf{C}_G(S)| = m^*(G)$ and since $G \in \CD(G)$, $|G|$ divides $m^*(G)$.  And so now we have that $G=ST$ is a direct product where $T$ is a Sylow $2$-subgroup of $\textbf{C}_G(S)$, which implies that $G$ is nilpotent, a contradiction.

So $X=G$, and the five subgroups not in $\CD(G)$ are the three Sylow $2$-subgroups, the identity subgroup, and $G$.

Let $T$ be a Sylow $2$-subgroup of $G$.  We argue that $|T|=2$.  Otherwise, there exists $1 < X \leq \textbf{Z}(T)$ with $X < T$, and so $X \in \CD(G)$.  Note that $m^*(G) = |X||\textbf{C}_G(X)| = |S||\textbf{C}_G(S)|$, and so $|S|$ divides $|\textbf{C}_G(X)|$.  And so $S \leq \textbf{C}_G(X)$ and so $X \leq \textbf{Z}(G) \leq S$, a contradiction (note $S$ contains $\textbf{Z}(G)$ since $S$ is in $\CD(G)$).

Hence $|T|=2$.  Note that $\textbf{C}_G(S)$ is a $3$-group as otherwise, since $|T|=2$, we would have a Sylow $2$-subgroup contained in $\textbf{C}_G(S)$, and hence $G$ is nilpotent, a contradiction.  And so $m^*(G) = |S||\textbf{C}_G(S)|$ is a power of $3$.  

Next, we argue that $T$ is self-normalizing.  Otherwise, let $Y$ be a Sylow $3$-subgroup of $\textbf{N}_G(T)$.  So $1 < Y < S$ (note that $Y < S$ as otherwise $S$ and $T$ would normalize one another, and so $G=ST$ would be nilpotent).  

But then $TY$ is a subgroup, and $T < TY < G$, and so $TY$ is in $\CD(G)$, which contradicts the fact that $m^*(G)$ is a power of $3$.

So $T$ is self-normalizing, and $3 = |G:\textbf{N}_G(T)| = |G:T| = |S|$.  So $S$ is cyclic of order $3$, $T$ is cyclic of order $2$, and $G = S_3$ with $\CD(G) = \{ S \}$ and, sure enough, $\delta_{ \CD }(G) = 5$.
\end{proof}
